Opportunities of a Machine Learning-based Decision Support System for Stroke Rehabilitation Assessment

Rehabilitation assessment is critical to determine an adequate intervention for a patient. However, the current practices of assessment mainly rely on therapist's experience, and assessment is infrequently executed due to the limited availability of a therapist. In this paper, we identified the needs of therapists to assess patient's functional abilities (e.g. alternative perspective on assessment with quantitative information on patient's exercise motions). As a result, we developed an intelligent decision support system that can identify salient features of assessment using reinforcement learning to assess the quality of motion and summarize patient specific analysis. We evaluated this system with seven therapists using the dataset from 15 patient performing three exercises. The evaluation demonstrates that our system is preferred over a traditional system without analysis while presenting more useful information and significantly increasing the agreement over therapists' evaluation from 0.6600 to 0.7108 F1-scores ($p <0.05$). We discuss the importance of presenting contextually relevant and salient information and adaptation to develop a human and machine collaborative decision making system.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> contents/evaluation-study.tex <==
\section{Evaluation Study}

==> contents/experiments.tex <==
\section{Experiments}\label{sect:experiments}
The main task of our experiments is to evaluate the quality of a motion (i.e. \textit{`correct'} and \textit{`incorrect'}) on three performance components for stroke rehabilitation. We collected the dataset of three stroke rehabilitation exercises from 15 post-stroke patients and 11 healthy subjects. We then evaluate how well our proposed method can align with the ground truth labels of therapist's evaluation while incorporating expert's domain knowledge. 
%The main goal of the experiments is to evaluate how well our proposed method can align with the ground truth scores of therapist's evaluation on patient's exercise motions. For the evaluation f the quality of a motion, we 
%What's the main goal?

%\subsubsection{Dataset}
\subsection{Data Collection}
\subsubsection{Exercise Motions} We recruited 15 stroke patients and 11 healthy subjects to collect the dataset of three upper limb exercises using a Kinect v2 sensor (Microsoft, Redmond, USA). The data collection program is implemented in C\# using Kinect SDK and Accord.NET framework \cite{de2014accord} and operated on a PC with 8GB RAM and i5-4590 3.3GHz 4 Cores CPU. This program records the 3D trajectory of joints and video frames at 30 Hz. The sensor was located at a height of 0.72m above the floor and 2.5m away from a subject. The starting and ending frames of exercise movements were manually annotated during the data collection.

Before participating in the data collection, all subjects signed the consent form. Fifteen post-stroke patients (13 males and 2 females) participated in two sessions for data collection: During the first session, a therapist evaluated post-stroke patient's functional ability using the a clinically validated tool, Fugl Meyer Assessment (FMA) (maximum score 66 points) \cite{sanford1993reliability}. 15 stroke survivors have diverse functional abilities from mild to severe impairment (37 $\pm$ 21 Fugl Meyer Scores). During the second session, a stroke survivor performed 10 repetitions of each exercise with both affected and unaffected sides. Eleven healthy subjects (10 males and 1 female) performed 15 repetitions with their dominant arms for each exercise. 
%Thus, we have 465 trials for each upper limb exercises. 165 trials of unaffected movements from 11 healthy subjects and 150 trials of affected movements from 15 post-stroke patients for training a prediction model. 150 trials of unaffected movements from 15 post-stroke patients are held out for training a user model. 

\textbf{\textit{`Training Data'}} (Figure \ref{fig:overall-arch}) is composed of 165 unaffected motions from 11 healthy subjects and 150 affected motions from 15 stroke survivors to train the Prediction Model (PM). 
\newline
\textbf{\textit{`User Data'}} (Figure \ref{fig:overall-arch}) includes each stroke survivor's unaffected motions for user-specific analysis of the visualization interface (Figure \ref{fig:web-interface}).

\subsubsection{Annotations for Implementing a Tool}
Therapist 1 (TP 1) had more interactions with recruited stroke patients by supporting the recruitment and evaluation on their functional ability with Fugl Meyer Assessment. Thus, we utilize therapist 1's annotations on the dataset to implement a system and evaluate it with other therapists (TP 3 - 9). Therapist 1 (TP1) watched the recorded videos of patient's movements (Figure \ref{fig:web-video}) and annotated exercise motion dataset using the scoring guideline (Table \ref{tab:score-guidelines}) without reviewing analysis of our system (Figure \ref{fig:web-traj}, \ref{fig:web-img}, \ref{fig:web-traj}).

%watch only videos without analysis 
%Therapist 1 (TP 1) supported to recruit stroke patients and evaluated their functional ability with the Fugl Meyer Assessment. 
%As Therapist 1 supported to recruit stroke patients and evaluated their functional ability with the Fugl Meyer Assessment, 
%We utilize Therapist 1's annotations on collected exercise motions to implement a system
%To implement a system for evaluation with another therapists (TP 3 - 9)
%We utilize the annotations of Therapists 1 to implement a tool for testing with another therapists (TP 3 - 9)
%As one therapist manages patient's rehabilitation from the beginning to the end for the consistent assessment and guidance and 
%the second evaluation of Therapist 1, who had more interactions with recruited patients as the ground truth labels.
%Two stroke rehabilitation therapists (i.e. Therapist 1 and Therapist 2 participated in two evaluation phases to generate annotations. Therapist 2 (TP 2) had no prior interactions with recruited patients. In the first phase, each therapist individually watched the recorded videos of patient's movements and annotated the correctness of performance components. In the second phase, two therapists had an one-hour discussion to share their evaluation strategies with one sample trial and then individually annotated the dataset again.
%Thus, the other therapist has better understanding of recrutied patients
%One therapist had no prior interactions with recruited patients. The other therapist supported to recruit stroke patients (Table \ref{tab:profile-post-stroke} and evaluated their functional ability with the FMA. We referre 


%\subsubsection{Additional Knowledge on Feature Relevance} Therapist 2 participated in the additional task of providing feature relevance to analyze the effect of accommodating therapist's knowledge on feature relevance. Therapist 2 reviewed 15 patient's user-specific analysis via the web interface (Figure \ref{fig:web-interface}) and generate the feature relevance whether a feature should be included or excluded to generate additional rules for assessment. 

%to include or exclude a feature
%To analyze the effect of accommodating additional therapist's knowledge on feature relevance, Therapist 2 reviewed 15 patient's user-specific analysis via the web interface. Therapists generated the feature relevance, whether to include or exclude to update 
%on each performance components of three exercises for 15 patients. 

%As a single therapist manages patient's rehabilitation from the beginning to the end for the consistent assessment and guidance, we utilized the evaluation of the primary therapist, who had more interactions with recruited patients as the ground truth scores. 

%Prediction Model 1 (PM 1) is an non-interactive, which does not utilizes any other information. PM 2 is an interactive, which utilize the domain knowledge of User

%W

%As a post-stroke survivor mainly interacts with a single therapist for the consistent assessment and guidance  \cite{rensink2009task, duncan2005management}, our study mainly explores how well our proposed method can be calibrated with the primary therapist's assessment and applicable to multiple patients.
 
%The overall procedure to measure agreement levels with the primary therapist is described in Figure \ref{fig:experiment-process}. We first measured the agreement between primary and secondary therapists during two evaluation phases, which can provide an idea of how well secondary therapist can align without or with one-hour discussion. We then computed the agreement levels between primary therapist and computer-assisted approaches (i.e. proposed and alternative approaches). Even if alternative approaches (i.e. multi-class classification and regression) are not shown in Figure \ref{fig:experiment-process}, we also computed their agreement levels using numerical ground truth of primary therapist's 2nd evaluation. We then compared agreement levels of the proposed approach with alternative approaches and secondary therapist to analyze any benefits of the proposed method.



%, which can be represented by joint angles or trajectory positions
%the discussion with therapists, we identified three commonly used factors 


%During a rehabilitation session, a patient performs task-oriented exercises to regain his/her functional ability and a therapist observes provides the assessment 

%The increasing prevalence of chronic diseases, such as heart failure, as the population ages is expected to result in a severe shortage in healthcare resources including nurses, physicians, and hospital beds [1], [2], [3]. Telemonitoring is a promising tool that can potentially alleviate some of the burden on the healthcare system by empowering patients to care for themselves and enabling more efficient clinical care, such as through automated alerts at the earliest sign of deteriorating patient health.






==> table/table-profiles-patients.tex <==
\begin{comment}
\begin{table}[h]
\centering
\caption{Profiles of 15 post-stroke survivors: }
\label{tab:profile-post-stroke}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{cccccccc} \toprule
\begin{tabular}[c]{@{}c@{}}Patient\\ ID\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total Fugl\\ (0-66)\end{tabular} & Age & Sex & \begin{tabular}[c]{@{}c@{}}Affected \\ Side\end{tabular} & Type \\ \midrule
P01 & 65 & 69 & M & Left & Not Specified \\
P02 & 65 & 60 & M & Left & Hemorphagic \\
P03 & 66 & 61 & M & Left & Not Specified \\
P04 & 66 & 63 & M & Right & Ischemic \\
P05 & 55 & 51 & M & Left & Ischemic \\
P06 & 13 & 63 & M & Left & Ischemic \& Spastic \\
P07 & 42 & 86 & F & Right & Ischemic \\
P08 & 15 & 71 & M & Left & Ischemic \\
P09 & 35 & 78 & M & Left & Hemorrphagic \\
P10 & 21 & 53 & M & Right & Ischemic \\
P11 & 16 & 37 & M & Right & Ischemic \\
P12 & 11 & 61 & M & Left & Hemorrphagic \\
P13 & 46 & 59 & M & Left & Ischemic \\
P14 & 11 & 67 & M & Left & Ischemic \\
P15 & 34 & 66 & F & Left & Ischemic \\ \bottomrule
\end{tabular}%
}
%\vspace{-1.0em}
\end{table}
\end{comment}
